Active Learning for Human-in-the-Loop Customs Inspection

We study the human-in-the-loop customs inspection scenario, where an AI-assisted algorithm supports customs officers by recommending a set of imported goods to be inspected. If the inspected items are fraudulent, the officers can levy extra duties. Th formed logs are then used as additional training data for successive iterations. Choosing to inspect suspicious items first leads to an immediate gain in customs revenue, yet such inspections may not bring new insights for learning dynamic traffic patterns. On the other hand, inspecting uncertain items can help acquire new knowledge, which will be used as a supplementary training resource to update the selection systems. Based on multiyear customs datasets obtained from three countries, we demonstrate that some degree of exploration is necessary to cope with domain shifts in trade data. The results show that a hybrid strategy of selecting likely fraudulent and uncertain items will eventually outperform the exploitation-only strategy.

==> tables/ablation_studies.tex <==
\begin{table}[ht!]
\centering
% \scriptsize
\caption{Results on the ablation study of the \update~ model.}
\label{tab:ablation_studies}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ l | c c  | c c  | c c } \toprule
    \multirow{2}{*}{} &
	\multicolumn{2}{c|}{$n=1\%$} & \multicolumn{2}{c|}{$n=5\%$} & \multicolumn{2}{c}{$n=10\%$} \\ \cmidrule{2-7}
	Model & \textsf{Pre.} & \textsf{Rev.} & \textsf{Pre.} & \textsf{Rev.} & \textsf{Pre.} & \textsf{Rev.} \\ \midrule
	\textbf{Full Model} & \textbf{92.66}\% & \textbf{44.97}\% & \textbf{38.77}\% & \textbf{84.35}\% & \textbf{20.24}\% & \textbf{89.03}\% \\
    \textbf{w/o MSA} & 91.83\% & 41.22\% & 38.47\%  & 82.64\% & 20.17\% & 86.34\%   \\
    \textbf{w/o FHI} & 89.89\% & 27.91\% & 36.03\%  & 80.39\% & 19.12\% & 78.79\%  \\
    \textbf{w/o DTL} & 90.72\% & 35.11\% &  37.57\%  & 78.46\%  & 19.74\%& 85.25\% \\ 
    \textbf{w/o AN} & 91.58\% & 40.20\%  &  38.11\% & 80.54\% & 19.02\% & 87.69\% \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/case_study.tex <==

\begin{table}[ht!]
\caption{Comparison of illicit and licit transaction $\mathbf{w.r.t}$ their corresponding cross features (CF) with highest attention score.}
\label{tab:case_study}
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cc}
\toprule
& Illicit case & Licit case\\ \midrule
Item & Used TOYOTA VENZA, \$16,863     & Used TOYOTA CAMRY, \$4,673 \\  \midrule
CF 1                  & \begin{tabular}[c]{@{}c@{}}risk.importer=0 \& tax.ratio\textless{}43.7\% \& \\ gross.weight\textless{}3327.43 \& fob.value\textgreater{}\$1,366\end{tabular} & 12.2\%\textless{}tax.ratio\textless{}16.8\% \& face.ratio\textgreater{}62.5\%  \\ \midrule
CF 2& \begin{tabular}[c]{@{}c@{}}value/kg\textgreater{}\$2 \& cif.value\textgreater{}\$1,912 \& \\ risk.(office,importer)=0 \& tax.ratio \textless{}0.18\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}risk.HS.origin=0 \& value/kg\textless{}\$2 \& \\ cif.value\textgreater{}\$1,640 \& risk.(office,importer)=0\end{tabular} \\ \midrule
$\hat{y}^{cls}$ & 0.9849 & 0.0001  \\ \bottomrule
\end{tabular}
}
\end{table}




% \begin{table}[!t]
% \caption{Description of significant cross features with higher attention weights in all illicit transactions. \sundong{Let's find some convincing example.}}
% \label{tab:case_study}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lc} \toprule
% Description of cross features & Attention weight or relevant score \\ \midrule
% Convincing cross feature 1  & 8 \\ 
% Convincing cross feature 2  & 4 \\ 
% Convincing cross feature 3 & 3 \\ 
% Convincing cross feature 4 & 2 \\ \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}[!t]
% \caption{Description of significant cross features with higher attention weights in all illicit transactions.}
% % \sundong{I will make it prettier. Roy, do you have any insight from this? Needs some descriptions, it looks like a cross feature generated by GBDT, how about \algo\'s attention + cross feature result? }
% % \roy{(The listed cross feature was obtained from the highest attention weight from our attention network. Considering there's 100 trees in our model and the limited space we have, it would be difficult to plot the attention weights and cross feature at the same time. )}
% \label{tab:case_study}
% \begin{tabular}{l|l}

% \hline
% ID   & Description of Cross Feature                                                                                                 \\ \hline
% $\mathbf{v_{749}}$  & \begin{tabular}[c]{@{}l@{}}{[}TaxRatio\textless{}0.2904{]} \& {[}CIF.VALUE\textgreater{}500053.5{]} \&\\ {[}Risk.IMPORTER=0{]}\end{tabular}                 \\ \hline
% $\mathbf{v_{800}}$  & \begin{tabular}[c]{@{}l@{}}{[}DayofYear\textgreater{}72{]} \& {[}CIF.VALUE\textgreater{}500048.5{]} \&\\ {[}Risk.OFFICE\&IMPORTER=0{]}\end{tabular} \\ \hline
% $\mathbf{v_{1072}}$ & {[}TaxRatio\textless{}0.0668{]} \& {[}FOBCIFRatio\textgreater{}0.625{]}                                                                                          \\ \hline
% $\mathbf{v_{1335}}$ & \begin{tabular}[c]{@{}l@{}}{[}Risk.HS6.Origin=0{]} \& {[}TARIFF.CODE\textless{}8.703e+09{]} \&\\ {[}Risk.QUANTITY=0{]}\end{tabular}                       \\ \hline
% \end{tabular}
% \end{table}

==> tables/corruption_rollback.tex <==
\begin{table}[t!]
\centering
% \scriptsize
\caption{Results on revised data by ~\algo.}
\label{tab:corruption-rollback}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ l | c c | c c | c c } \toprule
    \multirow{2}{*}{} &
	\multicolumn{2}{c|}{$n=1\%$} & \multicolumn{2}{c|}{$n=5\%$} & \multicolumn{2}{c}{$n=10\%$} \\ \cmidrule{2-7}
	Rescaling & \textsf{Pre.} & \textsf{Rev.} & \textsf{Pre.} & \textsf{Rev.} & \textsf{Pre.} & \textsf{Rev.} \\ \midrule
    \textbf{None} & 94.18\% & 44.55\% & 38.77\% & 83.98\% & 20.27\% & 89.30\%   \\
    \textbf{Deterministic} & 92.77\% & 44.80\% & 37.13\% & 77.69\% & 19.64\% & 84.41\%  \\
    \textbf{Stochastic} & 95.05\% & 42.38\% & 36.96\% & 77.11\% & 19.58\% & 83.90\% \\  \bottomrule
\end{tabular}
}
\end{table}



==> tables/exploration-exploitation-ratio.tex <==
\begin{table}[t!]
\centering
% \scriptsize
\caption{Performance difference by changing exploration-exploitation ratio}
\label{tab:datastats}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ l | l | l | l } \toprule
    Exploration ratio & Country M & Country N & Country T  \\ \midrule
    1\% & 0\% & 0\% & 0\%  \\ 
    2\% & 0\% & 0\% & 0\%  \\ 
    5\% & 0\% & 0\% & 0\%  \\ 
    10\% & 0\% & 0\% & 0\%  \\ 
    20\% & 0\% & 0\% & 0\%  \\ 
    30\% & 0\% & 0\% & 0\%  \\ 
    40\% & 0\% & 0\% & 0\%  \\ 
    50\% & 0\% & 0\% & 0\%  \\ 
    60\% & 0\% & 0\% & 0\%  \\ 
    70\% & 0\% & 0\% & 0\%  \\ 
    80\% & 0\% & 0\% & 0\%  \\ 
    90\% & 0\% & 0\% & 0\%  \\ 
    95\% & 0\% & 0\% & 0\%  \\ 
    98\% & 0\% & 0\% & 0\%  \\ 
    99\% & 0\% & 0\% & 0\%  \\  \bottomrule
\end{tabular}}
\end{table}

==> tables/main_results_selectivity_ratios.tex <==
\begin{table*}[t!]
\centering
\caption{Performance comparison between baselines and the proposed \algo.} \label{tab:main_results_selectivity_ratios}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ l | c c c | c c c | c c c | c c c | c c} \toprule
    \multirow{2}{*}{} &
	\multicolumn{3}{c|}{$n=1\%$ (Selecting top 1\%)} & \multicolumn{3}{c|}{$n=2\%$} & \multicolumn{3}{c|}{$n=5\%$} & \multicolumn{3}{c|}{$n=10\%$} & \multicolumn{2}{c}{Overall} \\ \cmidrule{2-15}
	Model & \textsf{Pre.}  & \textsf{Rec.} & \textsf{Rev.} & \textsf{Pre.}  & \textsf{Rec.} & \textsf{Rev.} & \textsf{Pre.}  & \textsf{Rec.} & \textsf{Rev.} & \textsf{Pre.}  & \textsf{Rec.} & \textsf{Rev.} & \textsf{AUC} & \textsf{F1} \\ \midrule
	\textsf{Price} & 2.75\% & 1.23\% & 15.17\% &  2.23\% & 1.99\% & 20.64\% & 2.06\% & 4.60\% & 34.95\% & 2.30\% & 10.28\% & 50.98\% & 67.57\% & 7.81\% \\
    \textsf{Importer} & 11.43\% & 5.10\% & 4.36\% &  9.41\% & 8.39\% & 7.56\% & 6.47\% & 14.43\% & 13.18\% & 5.22\% & 23.31\% & 30.31\% & 59.20\%  & 9.10\% \\
    \textsf{IForest} & 5.61\% & 2.50\% & 14.30\% &  6.19\% & 5.52\% & 23.14\% & 5.66\% & 12.62\% & 40.62\% & 5.12\% & 22.85\% & 54.14\% & 66.89\%  & 5.28\% \\
	\textsf{GBDT} & 90.01\% & 40.15\% &  24.59\% & 66.16\% & 59.04\% & 38.89\% & 32.19\% & 71.80\% & 57.20\% & 17.58\% & 78.42\% & 66.86\% & 93.38\% & 63.69\% \\
    \textsf{GBDT+LR} & 90.95\% & 40.40\% & 27.18\% & 72.94\% & 65.09\% & 44.22\% & 35.02\% & 78.11\% & 63.77\% & 18.72\% & 83.54\% & 73.77\% & 94.82\% & 68.76\% \\
    \textsf{TEM} &  88.72\% & 39.59\% & 39.48\% &  74.70\% & 66.43\% & 58.48\% & 37.39\% & 83.41\% & 78.58\% & 19.91\% & 88.54\% & 85.02\% & 96.52\% & 70.55\% \\ \midrule
    \textbf{\textsf{DATE\textsubscript{CLS}}} &  {\bf 92.66\%} & {\bf 41.33\%} & 44.97\% & {\bf 80.79\%} & {\bf 72.05\%} & 67.14\% & {\bf 38.77\%} & {\bf 86.49\%} & 84.35\% & {\bf 20.24\%} & {\bf 90.29\%} & 89.03\% & {\bf 96.79\%} & {\bf 75.32\%} \\ 
    \textbf{\textsf{DATE\textsubscript{REV}}} & 82.25\% & 36.63\% & {\bf 49.29\%} & 79.93\% & 71.22\% & {\bf 68.48\%} & 38.74\% & 86.41\% & {\bf 84.57\%} & 20.11\% & 89.74\% & {\bf 89.2\%} & 95.66\% & 75.23\% \\ 
    \bottomrule
\end{tabular}
}
\end{table*}

    % Improv. & -0.60\% & -0.29\% & 19.45\% &  6.22\% & 6.49\% & 16.01\% & 3.29\% & 3.27\% & 7.69\% & 2.01\% & 2.28\% & 5.95\% & 0.33\% & 6.38\% \\ 
    
    %% improvement from which baseline? the concept is value, so i removed, rather tahn I highlighted the best performance 
    
    % \sundong{Roy, I run \textsf{DATE\textsubscript{CLS}} and \textsf{DATE\textsubscript{REV}} 10 times, with l2=0.05, epoch=5. This is the averaged result.}



==> tables/test_on_subgroups.tex <==
\begin{table}[ht!]
\centering
\caption{Performance generated by \algocls~ on different subgroups of importers and HS codes in terms of various frequencies.}
\label{tab:subgroups}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ l | c c c | c c c | c } \toprule
    \multirow{2}{*}{} &
	\multicolumn{3}{c|}{$n=1\%$} & \multicolumn{3}{c|}{$n=5\%$} & \multirow{2}{*}{} \\ \cmidrule{2-7}
	Subgroup & \textsf{Pre.} & \textsf{Rec.} & \textsf{Rev.} & \textsf{Pre.} & \textsf{Rec.} & \textsf{Rev.} & Illicit rate \\ \midrule
    \textsf{Imp\textsubscript{$[0]$}} & 100.00\% & 39.27\% & 37.87\% & 45.72\% & 89.94\% & 87.41\% & 2.51\%  \\
    \textsf{Imp\textsubscript{$(0,10]$}} & 98.84\% & 41.47\% & 35.60\% & 42.44\% & 89.18\% & 81.57\% & 2.37\% \\
    \textsf{Imp\textsubscript{$(10,50]$}} & 98.86\% & 37.25\% & 35.44\% & 46.43\% & 87.46\% & 80.43\% & 2.65\% \\  
    \textsf{Imp\textsubscript{$(50,250]$}} & 91.72\% & 46.16\% & 38.64\% & 32.76\% & 82.31\% & 76.35\% & 1.99\% \\  
    \textsf{Imp\textsubscript{$(250,\infty)$}} & 72.76\% & 45.24\% & 53.10\% & 23.80\% & 73.90\% & 79.39\% & 1.60\% \\ \midrule
    \textsf{HS\textsubscript{$[0]$}} & 97.09\% & 27.52\% & 29.28\% & 51.21\% & 72.83\% & 70.66\% & 3.51\%  \\
    \textsf{HS\textsubscript{$(0,312]$}} & 91.50\% & 41.00\% & 53.74\% & 35.40\% & 79.35\% & 88.15\% & 2.23\% \\
    \textsf{HS\textsubscript{$(312,1781]$}} & 96.20\% & 44.48\% & 40.15\% & 39.45\% & 91.22\% & 84.08\% & 2.16\% \\  
    \textsf{HS\textsubscript{$(1781,8714]$}} & 98.19\% & 65.65\% & 54.79\% & 28.31\% & 94.67\% & 82.35\% & 1.49\% \\  
    \textsf{HS\textsubscript{$(8714,\infty)$}} & 99.81\% & 55.47\% & 56.21\% & 33.16\% & 92.16\% & 96.00\% & 1.17\% \\  
    \bottomrule
\end{tabular}
}
\end{table}

==> tables/type_of_customs_fraud.tex <==
\begin{table*}[!ht]
\caption{Types of customs fraud and the scope of this research}
    \centering
    %% begin table 
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}
    {@{}clll@{}}
        \toprule
            Covered
            & Fraud 
            & Description 
            & Illicit motives   \\ 
        \midrule
            \checkmark
            & \emph{Undervaluation} 
            & Declaration of trade goods 
            & to avoid customs duties and taxes;\\
            & \  &  with a lower price than the actual value 
            & to conceal illicit financial flows from exporters to importers \\ 
        \midrule
            \checkmark
            & \emph{Misclassification} 
            & Classification of trade goods 
            & to get a lower tariff rate applied; \\ 
            & \emph{of HS codes} 
            & into a wrong HS code 
            & to avoid prohibition/restriction applied to the correct HS code \\ 
        \midrule
            \checkmark
            & \emph{Manipulation of} 
            & Declaration of a false origin 
            & to get a preferential tariff rate \\ 
            & \emph{countries of origin} 
            & of trade goods 
            & under a free trade agreement \\ 
        \midrule
            & \emph{Smuggling} 
            & Trade of goods 
            & to avoid customs duties and taxes; \\ 
            & \ & without a customs declaration 
            & to avoid prohibition/restriction of the trade \\ 
        \midrule
            & \emph{Overvaluation} 
            & Declaration of trade goods 
            & to disguise illicit financial flows as legitimate trade-payment\\ 
            & \ & with a higher price than the actual value 
            &  (to conceal illicit financial flows from importers to exporters) \\ 
        \bottomrule
    \end{tabular}
    }
    \qquad
    %% begin figure 
    % \begin{minipage}[b]{0.3\textwidth}
    %     \includegraphics[width=0.99\columnwidth]{figures/customs-clearance}
    % \end{minipage}
% below is when we want separate captions
%\captionlistentry[table]{A table beside a figure}
%\captionsetup{labelformat=andtable}
\label{tab:types-fraud}
\end{table*}
